View N-gram Network for 3D Object Retrieval

How to aggregate multi-view representations of a 3D object into an informative and discriminative one remains a key challenge for multi-view 3D object retrieval. Existing methods either use view-wise pooling strategies which neglect the spatial information across different views or employ recurrent neural networks which may face the efficiency problem. To address these issues, we propose an effective and efficient framework called View N-gram Network (VNN). Inspired by n-gram models in natural language processing, VNN divides the view sequence into a set of visual n-grams, which involve overlapping consecutive view sub-sequences. By doing so, spatial information across multiple views is captured, which helps to learn a discriminative global embedding for each 3D object. Experiments on 3D shape retrieval benchmarks, including ModelNet10, ModelNet40 and ShapeNetCore55 datasets, demonstrate the superiority of our proposed method.

==> method.tex <==
\section{The proposed approach}
Given a 3D shape object $S$, we will first render it into a set of 2D greyscale view images, which is denoted by $V_{S} = \{v_1, v_2, ..., v_{|V|}\}$, where $v_j \in \mathbb{R}^{H \times W}$.  Our goal is to learn robust and discriminative 3D shape representations based on the rendered view set. An overview of our proposed architecture is shown in Fig.~\ref{fig:fig_arch}. As is presented, the whole model consists of 3 components, \ie~one shared \textbf{CNN1} that extracts features for each view image, The attentional feature enhancement and aggregation unit which applies N-gram feature enhancement over the view representations and then uses residual attention over the enhanced features. The last component the recognition part, which consists only one fully connected layer for recognition. 


\begin{figure*}
\includegraphics[width=\textwidth]{./Figures/model_crop.pdf}
\caption{The whole architecture of our proposed method. A shared CNN1 is used to extract features for each view images for 3D shape object. this Figure may be revised latter.}
\label{fig:fig_arch}
\end{figure*}
%-------------------------------------------------------------------------

\subsection{View Feature extraction}

For each rendered view images from 3D shape object, one shared convolutional neural network (CNN1) is used to extract its corresponding global high-level representations. This process can be formulated as 
\begin{align}
 \begin{split}
    & \mathbf{f}_i = \text{CNN1}(\mathbf{v}_i), i = 1, 2, 3, ..., |V|, 
\end{split}
\end{align}
where $\mathbf{f}_i\in\mathbb{R}^{d}$ represents the encoded feature vector of size $d$ for the i-th view image. Any existing
convolutional neural networks (\eg, AlexNet~\cite{ref},  VGG~\cite{ref}, GoogLeNet~\cite{ref}, ResNet~\cite{ref}) can be used for CNN1. In our work, we employ VGG11 with batch normalization, which is pretrained on ImageNet~\cite{ref}, as our backbone. The orginal VGG11 has 11 layers, which consists of 8 convolutional layers with convolutional kernel of size $3 \times 3$ and 3 fully connected layers. In our experiment, we remove the first two fully connected layer as our feature network. Therefore, each 3D shape can be represented multi-view embedding with the following form

\begin{equation}
 %\begin{split}
    \mathbf{F} = \mathbf{f}_1 \oplus \mathbf{f}_2 \oplus f_2 ...  \oplus \mathbf{f}_{|V|}
%\end{split}
\end{equation}

where $\oplus$ represents the concatenation operator, $\mathbf{F} \in \mathbb{R}^{|V| \times d}$ represents the encoded multi-view feature embedding matrix. 

%-------------------------------------------------------------------------
\subsection{Enhancing Multi-view Feature using N-gram Model}
%-------------------------------------------------------------------------
Traditional multi-view CNN perform max-pooling across the $V$ dimension, and feed the pooled representation to the latter layers of convolutional features for processing. However, it may cause information loss by maintaining only one maximum value at each position, which further leads to sub-optimal aggregated feature vector and hurt the performance. In our method, inspired by the N-gram model from natural language processing field, we can view each view image as one "word", and therefore one 3D shape object of $V$ view images can be  an analogy of one sentence of $|V|$ words. Therefore, for a 3D shape with $|V|$ view images, we can decompose the view sequence into a set of n-gram, and perform feature enhancement within each n-gram of view images.  This process can be seen as applies 2D convolutional kernel over the multi-view feature embedding matrix $\mathbf{F}$, which is formulated as 

\begin{equation}
\begin{split}
\mathbf{G} = \mathbf{F}  \circledast \mathcal{K}, sd =1
\end{split}
\end{equation}
where K is 2D convolutional kernel of size $n \times d$, and n is the number of gram considered. After this layer, we can obtain an enhanced features, where each row captures the information in each n-gram of view images. The idea behind the equation is illustrated in Fig.~\ref{??}

\subsection{Attentional Feature Aggregation}
%-------------------------------------------------------------------------
% maybe we need to state the motivate behind the attention mechanism. max pool drops much information, which might be useful for retrieval? Hence, we propose a better method to make use of as much information as possible from differnet views?

% \textcolor{blue}{Element-wise maximum operation is a widely adopted aggregation mechanism~\cite{} to produce more discriminative feature. However, }

To aggregate the n-gram enhanced features, we further propose to use an residual attentional feature aggregation unit. This unit first applies pooling operation to obtain a global descriptor for the 3D multiview representations, which is formulated as 
\begin{equation}
\begin{split}
\mathbf{f}_g = MaxPool(\mathbf{F})
\end{split}
\end{equation}

Therefore, based on $f_g$, we use this to compute an attention score for each enhanced features using dot product, 

\begin{equation}
\begin{split}
a_j = \frac{\exp(\mathbf{G_j} * \mathbf{f}_g)}{\sum_{i=1}^{|V|} \mathbf{G_j} * \mathbf{f}_g)}   
\end{split}
\end{equation}

Then we computed the attentional output over the enhanced view feature

\begin{equation}
\begin{split}
\mathbf{g}_{att} = \sum_{j=1}^{V+1-n} a_j \mathbf{g}_{i}    
\end{split}
\end{equation}

Finally, the attentional output is added to the max-pooling branch output using keronecker product, before they are fed into the layer normalization layer.   

\begin{equation}
\begin{split}
\mathbf{g}_{o} = LN(\mathbf{g}_{att} +  \mathbf{f}_g)  
\end{split}
\end{equation}
where $LN$ represents the layer normalization layer. Note that the above attentional process does not introduce any additional parameters.  

%-------------------------------------------------------------------------
We use softmax loss to train objective for our model, which is formulated as 

\begin{equation}
\label{eq:sft}
\begin{split}
L_{softmax} = & -\sum_{i=1}^{N} \log{Pr(y^i;W)} \\ & = -\sum_{i=1}^{bz} \log{ \frac{exp(W_{y_i}f_i + b_{y_i})}{\sum_{k=1}^{|\mathcal{Y}|} exp(W_{k}^T ) f_k + b_k}}
\end{split}
\end{equation}
where $f_i$ represents the input to the last fully connected layer of CNN2, which encodes the multi-view features for the i-th sample. $W_{k}$ represents the k-th column of the weights of the last fully connected layer, and $b_k$ represents the bias term. 

